Who Wrote this Code? Watermarking for Code Generation

Since the remarkable generation performance of large language models raised ethical and legal concerns, approaches to detect machine-generated text by embedding watermarks are being developed. However, we discover that the existing works fail to function appropriately in code generation tasks due to the task's nature of having low entropy. Extending a logit-modifying watermark method, we propose Selective WatErmarking via Entropy Thresholding (SWEET), which enhances detection ability and mitigates code quality degeneration by removing low-entropy segments at generating and detecting watermarks. Our experiments show that SWEET significantly improves code quality preservation while outperforming all baselines, including post-hoc detection methods, in detecting machine-generated code text. Our code is available in https://github.com/hongcheki/sweet-watermark.

==> resources_acl/fig_detectability.tex <==

\begin{figure}[t!]
\begin{center}
\includegraphics[width=\linewidth]{figure_acl/detectability_main.png}  
\end{center}
\caption{
\update{Detectability@T~\citep{kirchenbauer2023reliability} at HumanEval task. We set $\gamma=0.25$ and $\delta=3.0$ for $\wllm$ and $\myalgo$. For $\rdfw$, we use it with a high entropy setting. When calculating AUROC, we ensure at least 20 code texts of human-written solutions and machine-generated codes, respectively. We can observe that $\myalgo$ shows superior detection performance regardless of the text length.}
}\label{fig:detectability}
\end{figure}

==> resources_acl/table_rename.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{graphicx}
\begin{table}[]
\footnotesize
\resizebox{\columnwidth}{!}{%
\begin{tabular}{@{}llllll@{}}
\toprule
Method & 0\% & 25\% & 50\% & 75\% & 100\% \\ \midrule
$\rdfw$ & ??? & ??? & ??? & ??? & ??? \\
$\wllm$ & 0.925 & 0.890 & 0.846 & 0.792 & 0.738 \\
$\myalgo$ & 0.962 & 0.921 & 0.868 & 0.814 & 0.744 \\ \bottomrule
\end{tabular}%
}
\caption{AUROC values when detecting watermarking in the paraphrased source code. 0\% indicates the original watermarked code, and 100\% indicates that all variables are renamed. We conducted this experiment with five different random seeds and calculated the average AUROC values.}
\label{tab:rename_var}
\end{table}

==> sections/full_related_work.tex <==


\section{Related Work (Full ver.)}\label{sec:full_related_work}
%~\citep{zellers2019grover,OpenAI2023classifier}
\textbf{Post-hoc Text Detection.} There are numerous text detection methods where a simple classifier (e.g., logistic regression) is trained by identifying different characteristics in human-authored and machine-generated text. For example, GPTZero~\citep{tian2023gptzero} and Sniffer~\citep{li2023sniffer} focus on the difference in perplexity between human and LLM-written text. Ghostbuster~\citep{Verma2023Ghostbuster} and LLMDet~\citep{Wu2023LLMDet} uses the difference in probability-based features and n-gram-based proxy perplexity respectively. Another line of works uses pre-trained RoBERTa~\citep{Liu2019Roberta} and fine-tunes it as a classifier to identify the source of text~\cite{Solaiman2019Release,Ippolito2020Automatic,OpenAI2023classifier,Guo2023How,Yu2023GPT}. 
Although these training-based methods show impressive performance for in-domain text detection (i.e., the domain of testing text is similar to that of training data), they often lack generality for out-of-domain text. Moreover, the classifiers need to be consistently updated as new LLMs are continuously developed. 

Alternatively, another line of work tackle the detection problem without additional training procedure. GLTR~\citep{Gehrmann2019GLTR} focuses on the fact that machines generate each word from the head of their sampling distribution. The method compares the density or rank of each word in a given text to that of all possible candidates. \citet{Gehrmann2019GLTR} also proposes to measure the average log-rank of the tokens in the text and classifies it as model-generated if the log-rank is small. DetectGPT~\citep{Mitchell2023Detectgpt} observes that the machine-generated texts tend to lie at the local maximum of the log probability of LLMs. The method perturbs a given text in multiple ways and checks whether the log probability of a given text is higher than that of perturbed texts. DNA-GPT~\citep{Yang2023DNA} divides a given text in the middle and feeds only the first portion to the target LLM to generate various new remaining parts. Then the method compares the N-gram similarity between the original remaining part and the newly generated ones to identify the source of the text. These zero-shot methods often fail to detect texts generated by advanced LLMs, such as ChatGPT~\citep{OpenAI2022Chatgpt} and GPT-4~\citep{OpenAI2023gpt4}, and are limited to certain types of LLMs (e.g., decoder-only models). Furthermore, these methods heavily rely on multiple perturbations over LLM generations, which incurs huge computational costs.

\textbf{Text Watermarking.}
The majority of watermarking methods for text are based on the modification of the original text via a predefined set of rules \citep{Atallah2001Natural,Atallah2003Natural,Kim2003text,Topkara2006hiding,Jalil2009review,Meral2009Natural} or transformer-based networks \citep{Abdelnabi2021Adversarial,Yang2022Tracing,Yoo2023Robust}. However, there are only a few watermarking methods for LLMs that embed watermarks into tokens during the sampling process of LLMs. When the model samples each sentence, \citet{Venugopal2011Watermarking} proposed to generate a fixed number of candidates. A hash function is then applied to each candidate and generates a bit sequence from a binomial distribution with $p=0.5$ (i.e., the ratio of 0s and 1s is expected to be equal).  The watermarks are embedded by choosing candidates that are mapped to the bit sequences with the highest ratio of 1s. The difference in the ratio of 1s in the whole output is used to detect whether the output is watermarked or not. 

On the contrary, \citet{Kirchenbauer2023watermark} considered applying a hash function to the previously generated token, and uses the hash value as a seed for a random number generator to randomly divide candidate tokens into two groups. As the method induces sampling only from tokens belonging to one of the two groups (green and red), one with knowledge of this rule can detect the watermark if the output is generated by the model. 

We adopt the watermarking rule from ``soft watermark'' method in \citet{Kirchenbauer2023watermark}; however, our method differs from it in that we do not apply the rule to every single token when it is generated from a language model. In other words, while tokens with high entropy are sampled from the distribution biased to green list tokens, tokens with low entropy are from the original distribution, preserving the quality of the model outputs. Additionally, by preventing low entropy tokens from being watermarked, our selective method can reduce the number of red list tokens with such a high logit value that is inevitably generated. This affects much more effectively, especially in a code generation task, because a code block generated tends to be shorter than plain text, and the length of the text is critical for a statistical based detection method.

\textbf{Software Watermarking.}
One of the major streams of literature regarding watermarking code is software watermarking, which embeds a unique identifier within the code to protect the intellectual property of a software program. Based on the stage at which the watermarks are embedded, the methods are divided into static software watermarking \citep{Hamilton2011survey, Li2010Design,Myles2005evaluation}, which imprints watermarks in the codes of a software program, usually by code replacement and code re-ordering, and dynamic software watermarking \citep{Dey2019Software,Wang2018Exception,Ma2019Xmark}, which injects watermarks in the \textit{compiling/execution stage of a program}. These existing software watermarking methods not only differ from SWEET, but are not directly applicable to Code LLMs that are supposed to embed watermarks into the code during the generation process.
 


